LeakPair: Proactive Repairing of Memory Leaks in Single Page Web Applications

Modern web applications often resort to application development frameworks such as React, Vue.js, and Angular. While the frameworks facilitate the development of web applications with several useful components, they are inevitably vulnerable to unmanaged memory consumption since the frameworks often produce Single Page Applications (SPAs). Web applications can be alive for hours and days with behavior loops, in such cases, even a single memory leak in a SPA app can cause performance degradation on the client side. However, recent debugging techniques for web applications still focus on memory leak detection, which requires manual tasks and produces imprecise results. We propose LeakPair, a technique to repair memory leaks in single page applications. Given the insight that memory leaks are mostly non-functional bugs and fixing them might not change the behavior of an application, the technique is designed to proactively generate patches to fix memory leaks, without leak detection, which is often heavy and tedious. To generate effective patches, LeakPair follows the idea of pattern-based program repair since the automated repair strategy shows successful results in many recent studies. We evaluate the technique on more than 20 open-source projects without using explicit leak detection. The patches generated by our technique are also submitted to the projects as pull requests. The results show that LeakPair can generate effective patches to reduce memory consumption that are acceptable to developers. In addition, we execute the test suites given by the projects after applying the patches, and it turns out that the patches do not cause any functionality breakage; this might imply that LeakPair can generate non-intrusive patches for memory leaks.

==> table/rq4known.tex <==
\begin{table}[!t]
  \centering
	% \scriptsize
	\setlength\tabcolsep{2pt}
	\caption{Compilation results applying \toolname to the subjects in Table~\ref{tab:subject:known}.}
	\label{tab:compile:known}
	\resizebox{1.00\linewidth}{!}{%
\begin{threeparttable}
\begin{tabular}{c|c|c|c|c}
\toprule
ID &
Build/Compile Time Before LP Execution &
Build/Compile Time After LP Execution &
No. of Files &
LeakPair Execution Time
\\\midrule
K1 & 6407ms & 8742 ms & 47 & 3.5 s \\
2 & 6553 ms & 7337 ms & 4097 & 16.6 s \\
3 & 8485 ms & 5305 ms & 67 & 13.8 a \\
4 & 1 s & 0.6 s & 1921 & 8.9 s \\
5 & 167 ms & 110ms & 6083 & 10.9 s \\
6 & 9598 ms & 10529 ms & 117 & 4.2 s \\
7 & 10215 ms & 10242 ms & 1027 & 6 s \\
8 & 50 s & 51 s & 116 & 5 s \\
9 & 2758 ms & 2663 ms & 920 & 4 s \\
10 & 8319ms & 8319ms & 84 & 3.5 s
\\\bottomrule
\end{tabular}
{The full list of subjects used for our experiment is available in the replication package~\cite{}.}
\end{threeparttable}
}
\end{table}


==> table/rq4unknown.tex <==
\begin{table}[!t]
  \centering
	% \scriptsize
	\setlength\tabcolsep{2pt}
	\caption{Compilation results applying \toolname to the subjects in Table~\ref{tab:subject:unknown}.}
	\label{tab:compile:unknown}
	\resizebox{1.00\linewidth}{!}{%
\begin{threeparttable}
\begin{tabular}{c|c|c|c|c}
\toprule
ID &
Build/Compile Time Before LP Execution &
Build/Compile Time After LP Execution &
No. of Files &
LeakPair Execution Time \\
\midrule
U1 & 5395 ms & 6662 ms & 47 & 6.8 s \\
2 & 8597 ms & 8410 ms & 82 & 4.1 s \\
3 & 9503 ms & 8473 ms & 920 & 9.6s \\
4 & 3118 ms & 3851 ms & 124 & 7.1 s \\
5 & 5377 ms & 5433 ms & 78 & 19 s \\
6 & 37242 ms & 37242 ms & 277 & 3.2 s \\
7 & 3360 ms & 3713ms & 608 & 14.1 s \\
8 & 22831 ms & 21680 ms & 466 & 3.6 s \\
9 & 9.37 s & 9.18 s & 1122 & 13.1 s \\
10 & 9857ms & 10088ms & 999 & 5 s
\\\bottomrule
\end{tabular}
{The full list of subjects used for our experiment is available in the replication package~\cite{}.}
\end{threeparttable}
}
\end{table}

